Sequential Bayesian Optimization for Adaptive Informative Path Planning with Multimodal Sensing

Adaptive Informative Path Planning with Multimodal Sensing (AIPPMS) considers the problem of an agent equipped with multiple sensors, each with different sensing accuracy and energy costs. The agent's goal is to explore the environment and gather information subject to its resource constraints in unknown, partially observable environments. Previous work has focused on the less general Adaptive Informative Path Planning (AIPP) problem, which considers only the effect of the agent's movement on received observations. The AIPPMS problem adds additional complexity by requiring that the agent reasons jointly about the effects of sensing and movement while balancing resource constraints with information objectives. We formulate the AIPPMS problem as a belief Markov decision process with Gaussian process beliefs and solve it using a sequential Bayesian optimization approach with online planning. Our approach consistently outperforms previous AIPPMS solutions by more than doubling the average reward received in almost every experiment while also reducing the root-mean-square error in the environment belief by 50%. We completely open-source our implementation to aid in further development and comparison.

==> 4_Methods_old.tex <==

\subsection{Belief MDP Formulation} \label{sec:bmdp_formulation}
We formulate and solve the AIPPMS problem as a belief MDP in order to jointly reason about the effect of movement and multimodal sensing actions. The world environment is represented by a location graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ where the nodes $\mathcal{V}$ correspond to the set of all locations the agent can visit. The agent starts at $v_s$ and needs to reach a specified goal $v_g$ while remaining within its total cost budget $B$. The agent is equipped with a set of sensors with each sensor having a different cost and level of accuracy. We use notation consistent with previous work on the AIPP problem \cite{singh2009nonmyopic, choudhury2020adaptive}.

\textbf{Belief State Space $\mathcal{B}$}: The belief-state at time $t$ is defined as $b_t = (v_t, \Delta e_t, b_t(\mathcal{X}_\mathcal{V}))$ where $v_t$ is the agents current location and $\Delta e_t = B - \sum_{i=1}^{t-1} C(s_i, a_i)$ is the remainder of the cost budget where $C(s_i, a_i)$ is the cost associated with taking action $a_i$ from state $s_i$. Different costs are incurred for movement and sensing actions. Similarly, selecting a sensing action with greater accuracy will incur more cost than a sensing action with less accuracy. Note that the cost budget is different from the reward and is meant to track the energy resources of the agent. The problem terminates when the agent has too little energy left to take any actions which occurs when $\Delta e < \text{min}_a C(s_t,a)$. If the agent is not at the goal location $v_g$ when this happens it receives $-\infty$ reward. The world belief state $b(\mathcal{X}_\mathcal{V})$ is represented as a Gaussian process where $\mathcal{X}_\mathcal{V} \sim GP(m(\boldsymbol{x}), k(\boldsymbol{x}, \boldsymbol{x'}))$. 
    
\textbf{Action Space $\mathcal{A}$:} The action space is the union of all neighboring location states based on the current location and all sensing actions $\text{Nbrs}(v_t) \cup S$ where $S$ is the subspace of sensing actions.
    
\textbf{Transition Model $T$:} The transition function is fully deterministic for $v_t$ and $\Delta e_t$. If $a_t$ is a movement action to a neighboring node then $v_{t+1} = a_t$ and $\Delta e_{t+1} = \Delta e_{t} - C(s_t, a_{t+1})$. If $a_t$ is a sensing action then $v_{t+1} = v_t$ and the remaining cost budget will change accordingly. The transition for the world belief involves an update of the current belief state based on the result of any sampling actions taken. If a sampling action is taken, a measurement $y_t$ will be received at location $v_t$ and the Gaussian process update equations provided in Eq. \eqref{eq:gp_update} can be used to obtain the conditional posterior distribution $\boldsymbol{\hat{y}} \mid \boldsymbol{y_t}$ where $v_t$ is appended to the set of previously measured locations $\mathcal{X}_{\boldsymbol{y_t}}$ and $y_t$ is appended to the set of previously received measurements $\boldsymbol{y_t}$.
    
\textbf{Reward Function $R$:} 
The reward function is made up of two key elements. The first is the expected reward of interacting with the environment based on our current belief $\sum_s R(s,a)b(s)$. The second is based on the goal of minimizing the uncertainty in the world belief. To do so, we use the conditional entropy to evaluate the uncertainty in the world belief. We have that $\mathcal{X}_{\mathcal{V}}$ contains all of the locations in the environment and $\mathcal{X}_{\boldsymbol{y_t}}$ contains all of the locations that have been observed by the agent at time $t$. The goal is to minimize the conditional entropy of the environment based on the measurements received so far $\mathcal{X}_{\mathcal{V} \mid {\boldsymbol{y_{t-1}}}}$ given the new measurement location $\mathcal{X}_{\boldsymbol{y_t}}$. The conditional entropy is given by: 
\begin{gather} \label{eq:cond_entropy}
    \mathcal{H}(\mathcal{X}_{\mathcal{V} \mid {\boldsymbol{y_{t-1}}}} \mid \mathcal{X}_{\boldsymbol{y_t}}) = 
    \\ \nonumber - \int p(\mathcal{X}_{\mathcal{V} \mid {\boldsymbol{y_{t-1}}}}, \mathcal{X}_{\boldsymbol{y_t}}) \log p(\mathcal{X}_{\mathcal{V} \mid {\boldsymbol{y_{t-1}}}} \mid \mathcal{X}_{\boldsymbol{y_t}}) d \mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}} d \mathcal{X}_{\boldsymbol{y_t}}.
\end{gather} For a Gaussian process Eq. \eqref{eq:cond_entropy} is given by the analytical expression 
\begin{gather}
    \mathcal{H}(\mathcal{X}_{\mathcal{V} \mid {\boldsymbol{y_{t-1}}}} \mid \mathcal{X}_{\boldsymbol{y_t}}) = \frac{1}{2} \log \lvert \boldsymbol{\Sigma^{\ast}_{\mathcal{V} \mid y_t}} \rvert + \frac{D}{2} (1 + \log(2\pi)).
    \label{eq:analytical_cond_entropy}
\end{gather} 
As shown by Krause et al. minimizing the conditional entropy is equivalent to sampling at locations of highest entropy and for a Gaussian process, this is equivalent to sampling at locations with the greatest predictive variance \cite{krause2008near}. Similarly, sampling at locations with the greatest predictive variance is equivalent to sampling at locations that decrease the predictive variance the most. The predictive variance at each location in $\mathcal{X}_{\mathcal{V}}$ is given by the diagonals for the posterior covariance matrix $\Sigma^{\ast}$ so we seek to take the sequence of actions to maximally reduce the predictive variance, and thereby the conditional entropy, of the world belief state:
\begin{gather}
    \text{Tr} \left(\Sigma^{\ast}_{\mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}}} \right) - \text{Tr} \left( \Sigma^{\ast}_{\mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}} \mid \mathcal{X}_{\boldsymbol{y_t}}} \right).
    \label{eq:analytical_cond_entropy}
\end{gather}

% \begin{gather}
%     \nonumber \mathcal{H}(\mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}} \mid \mathcal{X}_{\boldsymbol{y_t}}) = 
%     \\ - \int p(\mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}}, \mathcal{X}_{\boldsymbol{y_t}}) \log p(\mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}} \mid \mathcal{X}_{\boldsymbol{y_t}}) d \mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}} d \mathcal{X}_{\boldsymbol{y_t}}.
%     \label{eq:cond_entropy}
% \end{gather}




% $\mathcal{H}(\mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}} \mid \mathcal{X}_{\boldsymbol{y_t}})$


% the mutual information. We have that $\mathcal{X}_{\mathcal{V}}$ contains all of the locations in the environment and $\mathcal{X}_{\boldsymbol{y_t}}$ contains all of the locations that have been observed by the agent at time $t$. The mutual information of the environment at unobserved locations $\mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}}$ given previously measured locations $\mathcal{X}_{\boldsymbol{y_t}}$ is 
% \begin{equation} \label{eq:mutual_information}
%     I(\mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}}; \mathcal{X}_{\boldsymbol{y_t}}) = \mathcal{H}(\mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}}) - \mathcal{H}(\mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}} \mid \mathcal{X}_{\boldsymbol{y_t}}) .
% \end{equation}
% where the conditional entropy of the unobserved locations $\mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}}$ after receiving measurements at locations $\mathcal{X}_{\boldsymbol{y_t}}$ is given by:



% \begin{gather}
%     \mathcal{H}(\mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}} \mid \mathcal{X}_{\boldsymbol{y_t}}) = \frac{1}{2} \log \sigma_{\mathcal{X}_{\mathcal{V} \setminus {\boldsymbol{y_t}}} \mid \mathcal{X}_{\boldsymbol{y_t}}}^2 + \frac{1}{2} (\log(2\pi) + 1)
%     \label{eq:analytical_cond_entropy}
% \end{gather}

% The mutual information at a belief state is equal to the expected reduction in belief entropy resulting from a measurement there. 
The belief-dependent reward function is then given by:

\begin{equation} \label{eq:reward}
        R(b, a, b') = \sum_s R(s,a)b(s) + \lambda I(\mathcal{X}_{\mathcal{V} \setminus y}; \mathcal{X}_y)
\end{equation} where $I(\mathcal{X}_{\mathcal{V} \setminus y}; \mathcal{X}_y)$ is the mutual information given by 



We set $\gamma = 1$


==> tables.tex <==

\\
text \\
text \\
text \\

\begin{tabular}{ ll | llll }
\toprule
     %& \multicolumn{1}{c|}{}  & & & & \\

    Budget & $\sigma_{s}$ & Random & GCB & MCTS-DPW & Raster \\
\hline   
    30 & 0.1 & & & & \\
    60 & 0.1 & & & & \\
    100 & 0.1 & & & & \\
    30 & 0.5 & & & & \\
    60 & 0.5 & & & & \\
    100 & 0.5 & & & & \\
    30 & 1.0 & & & & \\
    60 & 1.0 & & & & \\
    100 & 1.0 & & & & \\
\end{tabular}
\normalsize
\\
text \\
text \\
text \\

\begin{tabular}{ ll | llll }
\toprule
     %& \multicolumn{1}{c|}{}  & & & & \\

    Budget & $\sigma_{s}$ & Random & GCB & MCTS-DPW & Raster \\
\hline   
    30 & 0.1 & & & & \\
    30 & 0.5 & & & & \\
    30 & 1.0 & & & & \\
    60 & 0.1 & & & & \\
    60 & 0.5 & & & & \\
    60 & 1.0 & & & & \\
    100 & 0.1 & & & & \\
    100 & 0.5 & & & & \\
    100 & 1.0 & & & & \\
\end{tabular}
\normalsize
\\
text \\
text \\
text \\








% \begin{table*}[t]
% \begin{center}
% \label{table:results}
%     \begin{tabular}{@{}llllll@{}}
%     \toprule
%     %\multicolumn{7}{ c }{\textbf{Results}} \\
%     % \hline
%     %\midrule
%       & Rocks & Beacons & $p=0.5$ & $p=0.75$ & $p=1.0$ \\ 
%     \midrule

%     \bottomrule
%     \end{tabular}
%     \label{1}
% \end{center}
% \caption{Trajectories generated from the three different methods implemented. (a) and (b) MCTS. (c) and (d) MCTS-GSR. (e) and (f) ergodic control.}
% \end{table*}

% \begin{table*}[t]
% \begin{center}
% \label{table:results}
%     \begin{tabular}{@{}llllllll@{}}
%     \toprule
%     %\multicolumn{7}{ c }{\textbf{Results}} \\
%     % \hline
%     %\midrule
%       & Method & Iterations & Depth & K & Optimization Metric & Time (s) & Variance Reduction \\ 
%     \midrule
%     (a) & MCTS & 200 & 30 & -- & $R(b,a, b')$ & 292 & 4031 \\
%     (b) & MCTS & 300 & 50 & -- & $R(b,a, b')$ & 2549 & 3761 \\
%     (c) & MCTS-GSR & 300 & 300 & -- & $R(b)$ & 2641 & 3626 \\
%     (d) & MCTS-GSR & 1000 & 300 & -- & $R(b)$ & 9985 & 3522 \\
%     (e) & Ergodic & \textbf{71} & -- & 5 & \textbf{$\mathcal{E}$} & \textbf{4} &  4078\\ 
%     (f) & Ergodic & 74 & -- & 20 & $\mathcal{E}$ & 28 & 3835 \\ 
%     (g) & GP-PTO & 10000 & -- & -- & $R(b)$ & 5793 & 4435 \\ % this took the last one
%     (h) & \textbf{GP-PTO} & 10000 & -- & -- & $R(b)$ & 5761 & \textbf{4606} \\ % this selected the best from all iterations 
%     \bottomrule
%     \end{tabular}
%     \label{1}
% \end{center}
% \caption{Trajectories generated from the three different methods implemented. (a) and (b) MCTS. (c) and (d) MCTS-GSR. (e) and (f) ergodic control.}
% \end{table*}



text \\
text \\
text \\

\newpage 
\begin{tabular}{l|lllll}
\toprule
      & &\multicolumn{4}{c}{$\sigma_{s}=0.1$} \\
    \cline{2-6} \\
    Budget&& Random & GCB & MCTS-DPW & Raster \\
    \hline 
    30 & & & & & \\
    60 & & & & & \\
    100 & & & & & \\
\end{tabular}
\begin{tabular}{l|lllll}
\toprule
      & &\multicolumn{4}{c}{$\sigma_{s}=0.1$} \\
    \cline{2-6} \\
    Budget&& Random & GCB & MCTS-DPW & Raster \\
    \hline 
    30 & & & & & \\
    60 & & & & & \\
    100 & & & & & \\
\end{tabular}
\\
text \\
text \\
text \\

\begin{tabular}{l|lllll}
\toprule
      & &\multicolumn{4}{c}{$\sigma_{s}=0.1$} \\
    \cline{2-6} \\
    Budget&& Random & GCB & MCTS-DPW & Raster \\
    \hline 
    30 & & & & & \\
    60 & & & & & \\
    100 & & & & & \\
\hline 
    & &\multicolumn{4}{c}{$\sigma_{s}=0.5$} \\
    \cline{2-6} \\
     & & Random & GCB & MCTS-DPW & Raster \\
    \hline 
    30 & & & & & \\
    60 & & & & & \\
    100 & & & & & \\
\hline
    & &\multicolumn{4}{c}{$\sigma_{s}=1.0$} \\
    \cline{2-6} \\
     & & Random & GCB & MCTS-DPW & Raster \\
    \hline 
    30 & & & & & \\
    60 & & & & & \\
    100 & & & & & \\
\end{tabular}

% \begin{tabular}{ llllll}
% \toprule
%     & &\multicolumn{4}{c}{$\sigma_{s}=0.5$} \\
%     \cline{3-6} \\
%      & & Random & GCB & MCTS-DPW & Raster \\
%     \hline 
%     30 & & & & & \\
%     60 & & & & & \\
%     100 & & & & & \\
% \end{tabular}

% \begin{tabular}{llcccccc}

% \hline
% Rocks & Beacons &  $p=0.5$  & $p=0.75$  & $p=1.0$\\
% $k$ & $b$ & Random & GCB & Random & GCB & Random & GCB \\
% \cline{3-5}
% \\
% \cline{1--1}
% \\
% \textbf{Name} & \textbf{Country} & \textbf{Event} & \textbf{Result}\\\hline
% Anna-Karin Kammerling & Sweden & 50 m butterfly & 25.57\\ Wilson Kipketer & Denmark & 800 m & 2:11.96\\Jan Zelezný & Czech Republic & javelin throw & 98.5\\Sergei Bubka & Ukrain & pole vault & pole vault  \\ \hline
% \end{tabular}


% \begin{table*}[t]
% \begin{center}
% \label{table:results}
%     \begin{tabular}{@{}llllll@{}}
%     \toprule
%     %\multicolumn{7}{ c }{\textbf{Results}} \\
%     % \hline
%     %\midrule
%       & Rocks & Beacons & $p=0.5$ & $p=0.75$ & $p=1.0$ \\ 
%     \midrule

%     \bottomrule
%     \end{tabular}
%     \label{1}
% \end{center}
% \caption{Trajectories generated from the three different methods implemented. (a) and (b) MCTS. (c) and (d) MCTS-GSR. (e) and (f) ergodic control.}
% \end{table*}

